Generative Design of Hardware-aware DNNs

To efficiently run DNNs on the edge/cloud, many new DNN inference accelerators are being designed and deployed frequently. To enhance the resource efficiency of DNNs, model quantization is a widely-used approach. However, different accelerator/HW has different resources leading to the need for specialized quantization strategy of each HW. Moreover, using the same quantization for every layer may be sub-optimal, increasing the designspace of possible quantization choices. This makes manual-tuning infeasible. Recent work in automatically determining quantization for each layer is driven by optimization methods such as reinforcement learning. However, these approaches need re-training the RL for every new HW platform. We propose a new way for autonomous quantization and HW-aware tuning. We propose a generative model, AQGAN, which takes a target accuracy as the condition and generates a suite of quantization configurations. With the conditional generative model, the user can autonomously generate different configurations with different targets in inference time. Moreover, we propose a simplified HW-tuning flow, which uses the generative model to generate proposals and execute simple selection based on the HW resource budget, whose process is fast and interactive. We evaluate our model on five of the widely-used efficient models on the ImageNet dataset. We compare with existing uniform quantization and state-of-the-art autonomous quantization methods. Our generative model shows competitive achieved accuracy, however, with around two degrees less search cost for each design point. Our generative model shows the generated quantization configuration can lead to less than 3.5% error across all experiments.

==> sections/07-Discussion.tex <==
% \section{Discussion}

==> table/DIRECT.tex <==
\begin{table}
\centering
\caption{Comparisons with Naive Quantization}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline

 & mobilenet &  & resnet18 &  & resnet &  & mnasnet &  & proxylessnas &  \\ \hline
 & Memory & Accuracy & Memory & Accuracy & Memory & Accuracy & Memory & Accuracy & Memory & Accuracy \\ \hline
Direct (4) &  &  &  &  &  &  &  &  &  &  \\ \hline
Us &  &  &  &  &  &  &  &  &  &  \\ \hline
Direct (6) &  &  &  &  &  &  &  &  &  &  \\ \hline
Us &  &  &  &  &  &  &  &  &  &  \\ \hline
Direct (8) &  &  &  &  &  &  &  &  &  &  \\ \hline
Us &  &  &  &  &  &  &  &  &  &  \\ \hline
Original &  &  &  &  &  &  &  &  &  &  \\ \hline

\end{tabular}
\end{table}

==> table/HAQ.tex <==
\begin{table}
\centering
\caption{Comparison with HAQ}
\begin{tabular}{|l|l|l|l|l|}
\hline

 &  & cond 1 & Mean L1-loss & Search Time \\ \hline
mobilenetv2 & HAQ & 76\% & 0.19\% & 34 (min) \\ \hline
 & Ours & 76\% & 3.30\% & 1(min) \\ \hline
resnet18 & HAQ & 60\% & 0.00\% & 161(min) \\ \hline
 & Ours & 60\% & 2\% & 1(min) \\ \hline
mnasnet & HAQ & 69.4 & 1.61\% & 99 (min) \\ \hline
 & Ours & 66\% & 3\% & 1(min) \\ \hline
resnext & HAQ & N/A & N/A &  \\ \hline
 & Ours & 73\% & 3.50\% & 1(min) \\ \hline
proxylessnas & HAQ & N/A & N/A &  \\ \hline
 & Ours & 68\% & 2.70\% & 1(min) \\ \hline

\end{tabular}
\end{table}

==> table/PACT.tex <==
\begin{table}
\centering
\caption{Comparisons with DoReFa, PACT}
\begin{tabular}{|l|l|l|l|l|}
\hline

 & model & Memory & Accuracy & Search time \\ \hline
Dorefa (8) & mobilenet &  & 63.2 & 36 (min) \\ \hline
PACT (8) & mobilenet &  & 65.16 & 39 (min) \\ \hline
Ours & mobilenet &  &  &  \\ \hline
Dorefa (8) & Resnet18 &  & 71.6 & 36 (min) \\ \hline
PACT (8) & Resnet18 &  & 77.36 & 39 (min) \\ \hline
Ours & Resnet18 &  &  &  \\ \hline

\end{tabular}
\end{table}

==> table/alg.tex <==


\begin{algorithm}[tb]
   \caption{Pseudo code of training process}
   \label{alg:training}
\begin{algorithmic}
   \STATE {\bfseries Input:} I: number of iterations
   \FOR{$i=1$ {\bfseries to} $I-1$}
   \STATE \textbf{Sample} $m$ positive example \\$\left \{(c^{0}, x^{0}), (c^{1}, x^{1}),..., (c^{m-1}, x^{m-1})\right \}$
  \STATE  \textbf{Sample} $m$ noise sample $\left \{z^{0}, z^{1},..., z^{m-1}\right \}$, generate data $\left \{\tilde{x}^{0}, \tilde{x}^{2},..., \tilde{x}^{m-1}\right \}, \tilde{x}^{i}=G(c^{i}, z^{i})$ and reconstruct labels $\left \{\bar{c}^{0},\bar{c}^{1}...\bar{c}^{m-1}\right \}$ and $\left \{\tilde{c}^{0},\tilde{c}^{1}...\tilde{c}^{m-1}\right \}$, $\bar{c}^{i}=D_{2}(x^{})$, $\tilde{c}^{i}=D_{2}(\tilde{x}^{i})$
   \STATE \textbf{Update} discriminator V(D) via gradient ascent
   \STATE \textbf{Sample} $m$ noise sample, generated data and reconstruct labels 
   \STATE \textbf{Update} generator V(G) via gradient descent
   \STATE \textbf{Sample} $m$ noise sample, generated data and reconstruct labels 
   \STATE \textbf{Update} encoder V(E) via gradient descent
   \ENDFOR
\end{algorithmic}
\end{algorithm}


==> table/table2.tex <==
\begin{table}[h]
\centering
\caption{Comparisons with DoReDa and PACT}
\includegraphics[width=0.5\linewidth]{Figures/table2.pdf}
\vspace{-0.5cm}
\end{table}



